Millicharged Particles from the Heavens: Single- and Multiple-Scattering Signatures

For nearly a century, studying cosmic-ray air showers has driven progress in our understanding of elementary particle physics. In this work, we revisit the production of millicharged particles in these atmospheric showers and provide new constraints for XENON1T and Super-Kamiokande and new sensitivity estimates of current and future detectors, such as JUNO. We discuss distinct search strategies, specifically studies of single-energy-deposition events, where one electron in the detector receives a relatively large energy transfer, as well as multiple-scattering events consisting of (at least) two relatively small energy depositions. We demonstrate that these atmospheric search strategies -- especially this new, multiple-scattering signature -- provide significant room for improvement in the next decade, in a way that is complementary to anthropogenic, beam-based searches for MeV-GeV millicharged particles. Finally, we also discuss the implementation of a Monte Carlo simulation for millicharged particle detection in large-volume neutrino detectors, such as IceCube.

==> jdefs.tex <==
% Bibliography and bibfile
\def\pdu{Phys.\ Dark Univ.}
          % Physics of the Dark Universe
\def\lnp{Lec.\ Notes in Physics}
          % Lecture Notes in Physics
\def\cpc{Comp.\ Phys.\ Comm.}
          % Computer Physics Communications
\def\jpg{J. Phys. G}
          % Journal of Physics G Nuclear Physics
\def\ijmpa{Int.\ J.\ Mod.\ Phys.\ A}
          % International Journal of Modern Physics A
\def\epjc{Eur.\ Phys.\ J.\ C}
          % European Physical Journal C
\def\nima{Nuc.\ Inst.\ Methods A}
          % Nuclear Instruments and Methods A
\def\nimb{Nuc.\ Inst.\ Methods B}
          % Nuclear Instruments and Methods B
\def\njp{New J.\ Phys.}
          % New Journal of Physics
\def\rmp{Rev.\ Mod.\ Phys.}
          % Reviews of Modern Physics
\def\app{Astropart.\ Phys.}
          % Astroparticle Physics
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\arnps{Ann.~Rev.~Nucl.~\& Part.~Sci.}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.\ Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\pos{PoS}%
          % Proceedings of Science
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull.\ Astr.\ Inst.\ Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia
\def\caa{Chinese Astron.\ Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J.\ Astron.\ Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jhep{JHEP}%
          % Journal of High Energy Physics
\def\jcap{JCAP}%
          % Journal of Cosmology and Astroparticle Physics
\def\jinst{JINST}%
          % Journal of Instrumentation
\def\jpsj{J.\ Phys.\ Soc.\ Japan}%
          % Journal of the Physical Society of Japan
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\canjphys{Can.~J.~Phys.}
          %Canadian Journal of Physics
\def\apphys{Astropart.~Phys.}
          %Astroparticle Physics
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.\ Rev.\ A}%
          % Physical Review A: General Physics
\def\prb{Phys.\ Rev.\ B}%
          % Physical Review B: Solid State
\def\prc{Phys.\ Rev.\ C}%
          % Physical Review C
\def\prd{Phys.\ Rev.\ D}%
          % Physical Review D
\def\pre{Phys.\ Rev.\ E}%
          % Physical Review E
\def\prx{Phys.\ Rev.\ X}%
          % Physical Review X
\def\prl{Phys.\ Rev.\ Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.\ Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.\ Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\science{Science}%
\def\sci{\science}%
          % Science
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.\ Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.\ Space~Phys.\ Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.\ Astron.\ Inst.\ Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.\ Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.\ Cosmochim.\ Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.\ Res.\ Lett.}%
          % Geophysics Research Letters
\def\jcp{J.\ Chem.\ Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.\ Geophys.\ Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.\ Quant.\ Spec.\ Radiat.\ Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.\ Soc.\ Astron.\ Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.\ Phys.\ A}%
          % Nuclear Physics A
\def\nphysb{Nucl.\ Phys.\ B}%
          % Nuclear Physics B
\def\physrep{Phys.\ Rep.}%
          % Physics Reports
\def\physscr{Phys.\ Scr}%
          % Physica Scripta
\def\planss{Planet.\ Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.\ SPIE}%
          % Proceedings of the SPIE
\def\repprogphys{Rep.\ Prog.\ Phys.}%
          % Reports of Progress in Physics
\def\jpcrd{J. Phys. Chem. Ref. Data}%
        %Journal of Physical and Chemical Reference Data
\def\jphysb{J. Phys. B}%
	%Journal of Physics B Atomic Molecular Physics
\def\jphysd{J. Phys. D}%
	%Journal of Physics D
\def\jphysconfseries{J. Phys. Conf. Series}%
	%Journal of Physics: Conference Series
\def\physrev{\pr}
\def\pr{Phys. Rev.}%
	%Physical Review
\def\josa{J. Opt. Soc. Amer. (1917-1983)}%
	%Journal of the Optical Society of America (1917-1983)
\def\josab{J. Opt. Soc. Amer. B}%
	%Journal of the Optical Society of America B Optical Physics
\def\pla{Phys. Lett. A}%
	%Physics Letters A
\def\plb{Phys. Lett. B}%
	%Physics Letters B
\def\os{Opt. Spectrosc. (Russ.)}%
	%Optics and Spectroscopy (Russ. / USSR)
\def\jas{J. Appl. Spectrosc.}%
	%Journal of Applied Spectroscopy (Russ. / USSR)
\def\annp{Ann. Phys.}%
	%Annalen der Physik
\def\sa{Spectrochim. Acta}%
	%Spectrochimica Acta
\def\prsoca{Proc. R. Soc. London Ser. A}%
	%Proceedings of the Royal Society of London, Series A
\def\zphysa{Z. Phys. A}%
	%Zeitschrift fur Physik A
\def\zphysb{Z. Phys. B}%
	%Zeitschrift fur Physik B
\def\zphysc{Z. Phys. C}%
	%Zeitschrift fur Physik C
\def\zphysd{Z. Phys. D}%
	%Zeitschrift fur Physik D
\def\zphyse{Z. Phys. E}%
	%Zeitschrift fur Physik E
\def\zphys{Z. Phys.}%
	%Zeitschrift fur Physik
\def\adndt{Atom. Data Nuc. Data Tables}%
	%Atomic Data and Nuclear Data Tables
\def\jmolspec{J. Mol. Spectrosc.}%
	%Journal of Molecular Spectroscopy
\def\aphysb{Appl. Phys. B}%
	%Applied Physics B: Lasers and Optics
\def\nim{Nuc. Inst. Meth.}%
	%Nuclear Instruments and Methods
\def\jphysique{J. Phys. (Paris)}%
	%Journal de Physique
\def\epjp{Eur.~Phys.~J.~Plus}%
        %European Physical Journal Plus
\def\epjc{Eur.~Phys.~J.~C}%
        %European Physical Journal C
\def\epl{Europhys.~Lett}%
        %Europhysics Letters
\def\njp{New J.~Phys.}
        %New Journal of Physics
\def\statsci{StatSci}
\def\an{AstNach}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%


